Understanding the 2016 US Presidential Election using ecological inference and distribution regression with census microdata

We combine fine-grained spatially referenced census data with the vote outcomes from the 2016 US presidential election. Using this dataset, we perform ecological inference using distribution regression (Flaxman et al, KDD 2015) with a multinomial-logit regression so as to model the vote outcome Trump, Clinton, Other / Didn't vote as a function of demographic and socioeconomic features. Ecological inference allows us to estimate "exit poll" style results like what was Trump's support among white women, but for entirely novel categories. We also perform exploratory data analysis to understand which census variables are predictive of voting for Trump, voting for Clinton, or not voting for either. All of our methods are implemented in Python and R, and are available online for replication.

==> results/Age-Sex-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:43:04 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{5cm}lrrrrr}
  \hline
 &  Clinton & Trump & Frac& Part & Other / Non-voting \\
  \hline
 18 $<$= age $<$= 29 \& men & 0.55 & 0.45 & 0.08 & 0.39 & 0.61 \\ 
   18 $<$= age $<$= 29 \& women & 0.71 & 0.29 & 0.08 & 0.37 & 0.63 \\ 
   30 $<$= age $<$= 44 \& men & 0.43 & 0.57 & 0.13 & 0.56 & 0.44 \\ 
   30 $<$= age $<$= 44 \& women & 0.55 & 0.45 & 0.14 & 0.58 & 0.42 \\ 
   45 $<$= age $<$= 64 \& men & 0.48 & 0.52 & 0.16 & 0.49 & 0.51 \\ 
   45 $<$= age $<$= 64 \& women & 0.58 & 0.42 & 0.21 & 0.61 & 0.39 \\ 
   age $>$= 65 \& men & 0.36 & 0.64 & 0.10 & 0.57 & 0.43 \\ 
   age $>$= 65 \& women & 0.49 & 0.51 & 0.10 & 0.48 & 0.52 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Age-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:22 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\
  \hline
 18 $<$= age $<$= 29 & 0.62 & 0.38 & 0.17 & 0.42 & 0.58 \\ 
   30 $<$= age $<$= 44 & 0.54 & 0.46 & 0.25 & 0.54 & 0.46 \\ 
   45 $<$= age $<$= 64 & 0.46 & 0.54 & 0.39 & 0.58 & 0.42 \\ 
   age $>$= 65 & 0.45 & 0.55 & 0.18 & 0.47 & 0.53 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Citizenship-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:43:51 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{7cm}lp{1cm}rrrr}
  \hline
 & Clinton & Trump & Frac of elec & Part rate & Other / Non-voting \\ 
  \hline
 Born in the U.S. & 0.42 & 0.58 & 0.93 & 0.62 & 0.38 \\ 
   Born in Puerto Rico, Guam, the U.S. Virgin Islands, or the Northern Marianas
& 0.54 & 0.46 & 0.01 & 0.42 & 0.58 \\ 
   Born abroad of American parent(s) & 0.57 & 0.43 & 0.01 & 0.52 & 0.48 \\ 
   U.S. citizen by naturalization & 0.74 & 0.26 & 0.06 & 0.42 & 0.58 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Education-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:18 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\
  \hline
 High-school or less & 0.47 & 0.53 & 0.20 & 0.25 & 0.75 \\ 
   Some college & 0.46 & 0.54 & 0.33 & 0.49 & 0.51 \\ 
   Bachelor's degree & 0.51 & 0.49 & 0.30 & 0.84 & 0.16 \\ 
   Postgraduate education & 0.58 & 0.42 & 0.17 & 0.85 & 0.15 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Ethnicity-Sex-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 02:05:35 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 & Clinton & Trump & Fraction& Participation & Other \\ 
  \hline
 hispanic  men & 0.66 & 0.34 & 0.04 & 0.39 & 0.61 \\ 
   white  men & 0.39 & 0.61 & 0.36 & 0.57 & 0.43 \\ 
   black  men & 0.77 & 0.23 & 0.05 & 0.44 & 0.56 \\ 
   amerindian  men & 0.50 & 0.50 & 0.00 & 0.28 & 0.72 \\ 
   asian  men & 0.74 & 0.26 & 0.01 & 0.37 & 0.63 \\ 
   hispanic  women & 0.71 & 0.29 & 0.04 & 0.39 & 0.61 \\ 
   white  women & 0.48 & 0.52 & 0.38 & 0.57 & 0.43 \\ 
   black  women & 0.87 & 0.13 & 0.07 & 0.61 & 0.39 \\ 
   amerindian  women & 0.50 & 0.50 & 0.00 & 0.26 & 0.74 \\ 
   asian  women & 0.79 & 0.21 & 0.02 & 0.40 & 0.60 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Ethnicity-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 02:07:02 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 & Clinton & Trump & Fraction& Participation & Other \\ 
  \hline
 hispanic & 0.68 & 0.32 & 0.09 & 0.43 & 0.57 \\ 
   white & 0.40 & 0.60 & 0.72 & 0.54 & 0.46 \\ 
   black & 0.84 & 0.16 & 0.14 & 0.58 & 0.42 \\ 
   amerindian & 0.55 & 0.45 & 0.00 & 0.26 & 0.74 \\ 
   asian & 0.76 & 0.24 & 0.03 & 0.39 & 0.61 \\ 
   other/biracial & 0.76 & 0.24 & 0.01 & 0.34 & 0.66 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Income-Sex-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:43:42 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Frac & Part & Other / Non-voting \\
  \hline
 personal income $<$= 50000 \& men & 0.56 & 0.44 & 0.25 & 0.37 & 0.63 \\ 
   personal income $<$= 50000 \& women & 0.63 & 0.37 & 0.36 & 0.40 & 0.60 \\ 
   50000 $<$ personal income $<$= 100000 \& men & 0.40 & 0.60 & 0.15 & 0.67 & 0.33 \\ 
   50000 $<$ personal income $<$= 100000 \& women & 0.53 & 0.47 & 0.13 & 0.84 & 0.16 \\ 
   personal income $>$ 100000 \& men & 0.49 & 0.51 & 0.08 & 0.70 & 0.30 \\ 
   personal income $>$ 100000 \& women & 0.62 & 0.38 & 0.03 & 0.80 & 0.20 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Income-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:46:18 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{5cm}lrrrrr}
  \hline
 &  Clinton & Trump & Frac & Part & Other / Non-voting \\
  \hline
 personal income $<$= 50000 & 0.53 & 0.47 & 0.64 & 0.44 & 0.56 \\ 
   50000 $<$ personal income $<$= 100000 & 0.46 & 0.54 & 0.25 & 0.72 & 0.28 \\ 
   personal income $>$ 100000 & 0.45 & 0.55 & 0.11 & 0.77 & 0.23 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Misc-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:45:33 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{7cm}lrrrrr}
  \hline
 &  Clinton & Trump &  Part & Other / Non-voting \\
  \hline
 Language other than English spoken at home & 0.74 & 0.26 &  0.32 & 0.68 \\ 
  Mobility = lived here one year ago & 0.45 & 0.55 & 0.55 & 0.45 \\ 
  Mobility = moved here from outside US and Puerto Rico & 0.60 & 0.40 & 0.47 & 0.53 \\ 
  Mobility = moved here from inside US or Puerto Rico  & 0.56 & 0.44 & 0.48 & 0.52 \\ 
  Active duty military & 0.45 & 0.55 & 0.56 & 0.44 \\ 
  Not enrolled in school & 0.45 & 0.55 &  0.60 & 0.40 \\ 
  Enrolled in a public school or public college & 0.61 & 0.39 & 0.39 & 0.61 \\ 
  Enrolled in private school, private college, or home school & 0.66 & 0.34 & 0.53 & 0.47 \\ 
   \hline
\end{tabular}
\end{table}


==> results/MiscA-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 13:50:59 2016
\begin{table}[ht]
\centering
\begin{tabular}{rlrrrrr}
  \hline
 & subgroup & Clinton & Trump & Fraction.of.electorate & Participation.Rate & Other \\ 
  \hline
1 & LANX == 1 & 0.74 & 0.26 & 0.02 & 0.32 & 0.68 \\ 
  2 & MAR == 1 & 0.45 & 0.55 & 0.14 & 0.61 & 0.39 \\ 
  3 & MAR == 2 & 0.48 & 0.52 & 0.01 & 0.43 & 0.57 \\ 
  4 & MAR == 3 & 0.44 & 0.56 & 0.04 & 0.65 & 0.35 \\ 
  5 & MAR == 4 & 0.51 & 0.49 & 0.00 & 0.49 & 0.51 \\ 
  6 & MAR == 5 & 0.58 & 0.42 & 0.06 & 0.46 & 0.54 \\ 
  7 & MARHD == 1 & 0.44 & 0.56 & 0.00 & 0.57 & 0.43 \\ 
  8 & MARHM == 1 & 0.47 & 0.53 & 0.00 & 0.61 & 0.39 \\ 
  9 & MARHT == 1 & 0.44 & 0.56 & 0.14 & 0.59 & 0.41 \\ 
  10 & MARHT == 2 & 0.35 & 0.65 & 0.04 & 0.68 & 0.32 \\ 
  11 & MARHT == 3 & 0.27 & 0.73 & 0.01 & 0.59 & 0.41 \\ 
  12 & MIG == 1 & 0.45 & 0.55 & 0.22 & 0.55 & 0.45 \\ 
  13 & MIG == 2 & 0.60 & 0.40 & 0.00 & 0.47 & 0.53 \\ 
  14 & MIG == 3 & 0.56 & 0.44 & 0.03 & 0.48 & 0.52 \\ 
  15 & MIL == 1 & 0.45 & 0.55 & 0.00 & 0.56 & 0.44 \\ 
  16 & SCH == 1 & 0.45 & 0.55 & 0.25 & 0.60 & 0.40 \\ 
  17 & SCH == 2 & 0.61 & 0.39 & 0.02 & 0.39 & 0.61 \\ 
  18 & SCH == 3 & 0.66 & 0.34 & 0.01 & 0.53 & 0.47 \\ 
   \hline
\end{tabular}
\end{table}


==> results/Sex-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:23 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\ 
  \hline
Men  & 0.45 & 0.55 & 0.47 & 0.50 & 0.50 \\ 
  Women  & 0.56 & 0.44 & 0.53 & 0.53 & 0.47 \\ 
   \hline
\end{tabular}
\caption{Estimated demographic trends using our model. Columns show support for Clinton, Trump, 
fraction of the electorate made up by men (first row) vs women (second row), 
fraction of voting-age citizens who voted for Clinton or Trump,
and fraction of voting-age citizens who voted for a third party or did not vote.}
\label{table:sex}
\end{table}


==> results/Socio-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:46:16 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{7cm}lrrrrr}
  \hline
 &  Clinton & Trump & Part.& Other / Non-voting \\
  \hline
 Hearing difficulty & 0.37 & 0.63  & 0.47 & 0.53 \\ 
   Vision difficulty & 0.42 & 0.58  & 0.46 & 0.54 \\ 
   Independent living difficulty & 0.50 & 0.50  & 0.28 & 0.72 \\ 
   Veteran service connected disability rating (percentage) $\geq$ 10\% & 0.07 & 0.93  & 0.82 & 0.18 \\ 
   Cognitive difficulty & 0.52 & 0.48  & 0.23 & 0.77 \\ 
   Ability to speak English = well & 0.73 & 0.27  & 0.31 & 0.69 \\ 
   Ability to speak English = not well or not at all  & 0.67 & 0.33  & 0.21 & 0.79 \\ 
   Gave birth to a child within the past 12 months & 0.51 & 0.49  & 0.64 & 0.36 \\ 
   Grandparents living with grandchildren & 0.46 & 0.54  & 0.44 & 0.56 \\ 
  Grandparents responsible for grandchildren & 0.42 & 0.58  & 0.53 & 0.47 \\ 
 Insurance purchased directly from an insurance company  & 0.43 & 0.57  & 0.59 & 0.41 \\ 
  Medicare, for people 65 and older, or people with certain disabilities & 0.44 & 0.56  & 0.46 & 0.54 \\ 
  Medicaid or similar & 0.56 & 0.44  & 0.27 & 0.73 \\ 
  TRICARE or other military health care & 0.26 & 0.74  & 0.72 & 0.28 \\ 
  VA used ever & 0.21 & 0.79  & 0.70 & 0.30 \\ 
  Indian Health Service  & 0.69 & 0.31  & 0.22 & 0.78 \\ 
   \hline
\end{tabular}
\end{table}


==> results/bigtable.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:23 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\ 
  \hline
Men  & 0.45 & 0.55 & 0.47 & 0.50 & 0.50 \\ 
  Women  & 0.56 & 0.44 & 0.53 & 0.53 & 0.47 \\ 
   \hline
  \hline
 18--29 year olds & 0.62 & 0.38 & 0.17 & 0.42 & 0.58 \\ 
   30--44 & 0.54 & 0.46 & 0.25 & 0.54 & 0.46 \\ 
   45--64 & 0.46 & 0.54 & 0.39 & 0.58 & 0.42 \\ 
   65  and older & 0.45 & 0.55 & 0.18 & 0.47 & 0.53 \\ 
   \hline
\end{tabular}
\caption{Estimated demographic trends using our model. Columns show support for Clinton, Trump, 
fraction of the electorate made up by men (first row) vs women (second row), 
fraction of voting-age citizens who voted for Clinton or Trump,
and fraction of voting-age citizens who voted for a third party or did not vote.}
\label{table:sex}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{p{5cm}rrp{2cm}p{2cm}r}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\\hline
  Educational attainment & & & & & \\ 
  \hline
 High-school or less & 0.47 & 0.53 & 0.20 & 0.25 & 0.75 \\ 
   Some college & 0.46 & 0.54 & 0.33 & 0.49 & 0.51 \\ 
   Bachelor's degree & 0.51 & 0.49 & 0.30 & 0.84 & 0.16 \\ 
   Postgraduate education & 0.58 & 0.42 & 0.17 & 0.85 & 0.15 \\ 
   \hline
   \hline
  Race/Ethnicity & & & & & \\ 
  \hline
 hispanic & 0.68 & 0.32 & 0.09 & 0.43 & 0.57 \\ 
   white & 0.40 & 0.60 & 0.72 & 0.54 & 0.46 \\ 
   black & 0.84 & 0.16 & 0.14 & 0.58 & 0.42 \\ 
   asian & 0.76 & 0.24 & 0.03 & 0.39 & 0.61 \\ 
   \hline
   \hline
  Place of birth & & & & & \\ 
  \hline
 Born in the U.S. & 0.42 & 0.58 & 0.93 & 0.62 & 0.38 \\ 
   U.S. citizen by naturalization & 0.74 & 0.26 & 0.06 & 0.42 & 0.58 \\ 
   \hline
  \hline
  Personal income & & & & & \\ 
  \hline
 below \$50,000 & 0.53 & 0.47 & 0.64 & 0.44 & 0.56 \\ 
   \$50,000 to \$100,000 & 0.46 & 0.54 & 0.25 & 0.72 & 0.28 \\ 
   more than \$100,000 & 0.45 & 0.55 & 0.11 & 0.77 & 0.23 \\ 
   \hline
\end{tabular}
\caption{Estimated demographic trends using our model for various census variables. Columns show support for Clinton, Trump, 
fraction of the electorate made up by men (first row) vs women (second row), 
fraction of voting-age citizens who voted for Clinton or Trump,
and fraction of voting-age citizens who voted for a third party or did not vote.}
\label{table:other}
\end{table}


==> results/deviance.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 02:45:56 2016
\begin{table}[ht]
\centering
\begin{tabular}{rlrr}
  \hline
 & feature & deviance & frac.deviance \\ 
  \hline
1 & RAC3P - race coding & 0.04 & 0.86 \\ 
  2 & ethnicity interacted with has degree& 0.04 & 0.74 \\ 
  3 & schooling attainment & 0.04 & 0.72 \\ 
  4 & ANC2P - detailed ancestry & 0.04 & 0.83 \\ 
  5 & OCCP - occupation & 0.04 & 0.75 \\ 
  6 & COW - class of worker & 0.04 & 0.67 \\ 
  7 & ANC1P - detailed ancestry & 0.05 & 0.77 \\ 
  8 & NAICSP - industry code & 0.05 & 0.71 \\ 
  9 & RAC2P - race code & 0.05 & 0.70 \\ 
  10 & age interacted with usual hours worked per week (WKHP) & 0.05 & 0.69 \\ 
  11 & sex interacted with ethnicity& 0.05 & 0.65 \\ 
  12 & MSP - marital status& 0.05 & 0.61 \\ 
  13 & FOD1P - field of degree & 0.05 & 0.61 \\ 
  14 & ethnicity & 0.06 & 0.57 \\ 
  15 & RAC1P - recoded race & 0.06 & 0.54 \\ 
  16 & sex interacted with age & 0.06 & 0.57 \\ 
  17 & has degree interacted with age & 0.06 & 0.55 \\ 
  18 & age interacted with personal income & 0.06 & 0.76 \\ 
  19 & sex interacted with hours worked per week  & 0.06 & 0.62 \\ 
  20 & personal income interacted with hours worked per week & 0.06 & 0.69 \\ 
  21 & personal income& 0.06 & 0.59 \\ 
  22 & RACSOR - single or multiple race & 0.07 & 0.42 \\ 
  23 & has degree interacted with hours worked per week & 0.07 & 0.59 \\ 
  24 & hispanic & 0.07 & 0.56 \\ 
  25 & sex interacted with personal income & 0.07 & 0.57 \\ 
   \hline
\end{tabular}
\caption{Lower deviance values indicate a better fit. Larger fraction of deviance explained values are better. Models are fit to the outcome data as described
in the text using only the categorical predictors or interactions of
categorical predictors listed.}
\label{table:deviance}
\end{table}


==> tables/Age-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:22 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\
  \hline
 18 $<$= age $<$= 29 & 0.62 & 0.38 & 0.17 & 0.42 & 0.58 \\ 
   30 $<$= age $<$= 44 & 0.54 & 0.46 & 0.25 & 0.54 & 0.46 \\ 
   45 $<$= age $<$= 64 & 0.46 & 0.54 & 0.39 & 0.58 & 0.42 \\ 
   age $>$= 65 & 0.45 & 0.55 & 0.18 & 0.47 & 0.53 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Citizenship-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:43:51 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{7cm}lp{1cm}rrrr}
  \hline
 & Clinton & Trump & Frac of elec & Part rate & Other / Non-voting \\ 
  \hline
 Born in the U.S. & 0.42 & 0.58 & 0.93 & 0.62 & 0.38 \\ 
   Born in Puerto Rico, Guam, the U.S. Virgin Islands, or the Northern Marianas
& 0.54 & 0.46 & 0.01 & 0.42 & 0.58 \\ 
   Born abroad of American parent(s) & 0.57 & 0.43 & 0.01 & 0.52 & 0.48 \\ 
   U.S. citizen by naturalization & 0.74 & 0.26 & 0.06 & 0.42 & 0.58 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Education-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:18 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\
  \hline
 High-school or less & 0.47 & 0.53 & 0.20 & 0.25 & 0.75 \\ 
   Some college & 0.46 & 0.54 & 0.33 & 0.49 & 0.51 \\ 
   Bachelor's degree & 0.51 & 0.49 & 0.30 & 0.84 & 0.16 \\ 
   Postgraduate education & 0.58 & 0.42 & 0.17 & 0.85 & 0.15 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Ethnicity-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 02:07:02 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 & Clinton & Trump & Fraction& Participation & Other \\ 
  \hline
 hispanic & 0.68 & 0.32 & 0.09 & 0.43 & 0.57 \\ 
   white & 0.40 & 0.60 & 0.72 & 0.54 & 0.46 \\ 
   black & 0.84 & 0.16 & 0.14 & 0.58 & 0.42 \\ 
   amerindian & 0.55 & 0.45 & 0.00 & 0.26 & 0.74 \\ 
   asian & 0.76 & 0.24 & 0.03 & 0.39 & 0.61 \\ 
   other/biracial & 0.76 & 0.24 & 0.01 & 0.34 & 0.66 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Income-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:46:18 2016
\begin{table}[ht]
\centering
\begin{tabular}{p{5cm}lrrrrr}
  \hline
 &  Clinton & Trump & Frac & Part & Other / Non-voting \\
  \hline
 personal income $<$= 50000 & 0.53 & 0.47 & 0.64 & 0.44 & 0.56 \\ 
   50000 $<$ personal income $<$= 100000 & 0.46 & 0.54 & 0.25 & 0.72 & 0.28 \\ 
   personal income $>$ 100000 & 0.45 & 0.55 & 0.11 & 0.77 & 0.23 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/MiscA-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 13:50:59 2016
\begin{table}[ht]
\centering
\begin{tabular}{rlrrrrr}
  \hline
 & subgroup & Clinton & Trump & Fraction.of.electorate & Participation.Rate & Other \\ 
  \hline
1 & LANX == 1 & 0.74 & 0.26 & 0.02 & 0.32 & 0.68 \\ 
  2 & MAR == 1 & 0.45 & 0.55 & 0.14 & 0.61 & 0.39 \\ 
  3 & MAR == 2 & 0.48 & 0.52 & 0.01 & 0.43 & 0.57 \\ 
  4 & MAR == 3 & 0.44 & 0.56 & 0.04 & 0.65 & 0.35 \\ 
  5 & MAR == 4 & 0.51 & 0.49 & 0.00 & 0.49 & 0.51 \\ 
  6 & MAR == 5 & 0.58 & 0.42 & 0.06 & 0.46 & 0.54 \\ 
  7 & MARHD == 1 & 0.44 & 0.56 & 0.00 & 0.57 & 0.43 \\ 
  8 & MARHM == 1 & 0.47 & 0.53 & 0.00 & 0.61 & 0.39 \\ 
  9 & MARHT == 1 & 0.44 & 0.56 & 0.14 & 0.59 & 0.41 \\ 
  10 & MARHT == 2 & 0.35 & 0.65 & 0.04 & 0.68 & 0.32 \\ 
  11 & MARHT == 3 & 0.27 & 0.73 & 0.01 & 0.59 & 0.41 \\ 
  12 & MIG == 1 & 0.45 & 0.55 & 0.22 & 0.55 & 0.45 \\ 
  13 & MIG == 2 & 0.60 & 0.40 & 0.00 & 0.47 & 0.53 \\ 
  14 & MIG == 3 & 0.56 & 0.44 & 0.03 & 0.48 & 0.52 \\ 
  15 & MIL == 1 & 0.45 & 0.55 & 0.00 & 0.56 & 0.44 \\ 
  16 & SCH == 1 & 0.45 & 0.55 & 0.25 & 0.60 & 0.40 \\ 
  17 & SCH == 2 & 0.61 & 0.39 & 0.02 & 0.39 & 0.61 \\ 
  18 & SCH == 3 & 0.66 & 0.34 & 0.01 & 0.53 & 0.47 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Sex-national.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Nov 10 00:42:23 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 &  Clinton & Trump & Fraction of electorate & Participation Rate & Other / Non-voting \\ 
  \hline
Men  & 0.45 & 0.55 & 0.47 & 0.50 & 0.50 \\ 
  Women  & 0.56 & 0.44 & 0.53 & 0.53 & 0.47 \\ 
   \hline
\end{tabular}
\caption{Estimated demographic trends using our model. Columns show support for Clinton, Trump, 
fraction of the electorate made up by men (first row) vs women (second row), 
fraction of voting-age citizens who voted for Clinton or Trump,
and fraction of voting-age citizens who voted for a third party or did not vote.}
\label{table:sex}
\end{table}

